Recurrent Feedback Improves Feedforward Representations in Deep Neural Networks

The abundant recurrent horizontal and feedback connections in the primate visual cortex are thought to play an important role in bringing global and semantic contextual information to early visual areas during perceptual inference, helping to resolve local ambiguity and fill in missing details. In this study, we find that introducing feedback loops and horizontal recurrent connections to a deep convolution neural network (VGG16) allows the network to become more robust against noise and occlusion during inference, even in the initial feedforward pass. This suggests that recurrent feedback and contextual modulation transform the feedforward representations of the network in a meaningful and interesting way. We study the population codes of neurons in the network, before and after learning with feedback, and find that learning with feedback yielded an increase in discriminability (measured by d-prime) between the different object classes in the population codes of the neurons in the feedforward path, even at the earliest layer that receives feedback. We find that recurrent feedback, by injecting top-down semantic meaning to the population activities, helps the network learn better feedforward paths to robustly map noisy image patches to the latent representations corresponding to important visual concepts of each object class, resulting in greater robustness of the network against noises and occlusion as well as better fine-grained recognition.

==> sections/left.tex <==
\begin{table*}
\capbtabbox{
  \begin{tabular}{l|c|c|c|c|c}
  \toprule
  \cmidrule(r){1-2}
  \diagbox{Noise Level}{Models} & VGG16 & Module 1 & Module 2 & Module 3 & Proposed \\
  \midrule
  0 & 71.076 & 71.608 & 71.540 & 71.500 & \textbf{71.632} \\
  10 & 65.456 & 66.400 & 66.578 & 66.580 & \textbf{66.760} \\
  20 & 54.090 & 56.630 & 55.944 & 56.040 & \textbf{56.294} \\
  30 & 39.124 & 41.090 & 41.800 & 41.520 & \textbf{42.104} \\
  40 & 24.068 & 26.980 & 27.634 & 26.910 & \textbf{27.766} \\
  50 & 13.072 & 15.890 & \textbf{16.458} & 15.460 & 16.310 \\
  \bottomrule
  \end{tabular}
}{
 \caption{Noise image classification top-1 accuracy on different module structures. VGG16: standard feedforward model. module 1: top-down gating contextual. module 2: contextual gating contextual. module 3: contextual gating top-down and top-down gating contextual combined. Proposed: contextual gating top-down.}
 \label{tab:diff-model}
}
\end{table*}

\begin{table*}
\capbtabbox{
  \begin{tabular}{l|c|c|c|c|c}
  \toprule
  \cmidrule(r){1-2}
  Models & Imagenet \\
  \midrule
  VGG16 \citep{simonyan2014very} & 71.076\\
  VGG-LR-2 \citep{li2018learning} & 71.551 \\
  VGG-GCM-4 & \textbf{71.741}\\
  \bottomrule
  \end{tabular}
}{
 \caption{ImageNet classification top-1 accuracy.}
 \label{tab:imagenet-top1}
}
\end{table*}

\begin{figure}
\begin{floatrow}
\capbtabbox{%
  \begin{tabular}{|l|c|c|}
  \toprule
  \cmidrule(r){1-2}
  Model & CUB-200\\
  \midrule
  VGG-small & 64.88\\
  %VGG-ATT \citep{jetley2018learn} & 73.19 \\
  VGG-LR-2 \citep{li2018learning} & 72.99 \\ 
  %ResNet-34 \citep{he2016deep} & 73.50 \\
  VGG-CRCN-4 & \textbf{74.91}\\
  \bottomrule
  \end{tabular}
}{%
 \caption{Top-1 accuracy on CUB-200 datasets.}
 \label{tab:cub}
}
\capbtabbox{%
  \begin{tabular}{|l|c|}
  \toprule
  \cmidrule(r){1-2}
  Model & Occlusion\\
  \midrule
  VGG-small & 34.50\\
  %VGG-ATT \citep{jetley2018learn} & 46.57 \\
  VGG-LR-2 \citep{li2018learning} & 45.88 \\
  VGG-CRCN-4 & \textbf{50.72}\\
  \bottomrule
  \end{tabular}
}{%
 \caption{Top-1 accuracy on Occlusion datasets.}
 \label{tab:occlusion}
}
\end{floatrow}
\end{figure}

\begin{figure}[htb]
\centering
  \includegraphics[width=\textwidth]{Figures/noise_level.png}
  \caption{The example images and results of noise image classification experiment. Upper four images show an example of images with different levels of Gaussian noise added. From left to right, the  standard deviations are 0, 10, 30, 50, respectively. Lower right figure shows the increased percentage of our unroll-2-times model on top-1 noise image accuracy compared with feedforward model. Lower left figure shows the adversarial attack result. The fooling rate is measured by the absolute accuracy drop when adversarial attack is performed on the model. We use standard FGSM attack on all ImageNet validation images. The blue line shows the fooling rate of our unroll-2-times model, red line shows the feed-forward model and the orange line shows the model proposed by \citep{li2018learning}. As the attack gets stronger, our model shows more robustness.}
  \label{fig:noise_inte}
\end{figure}

\author{Siming Yan*, Bowen Xiao* \\
Department of Computer Science\\
Peking University\\
Beijing 100871, China \\
\texttt{\{simingyan,mike.xiao\}@pku.edu.cn} \\
\And
Yimeng Zhang, Tai-Sing Lee \\
Department of Computer Science\\
Carnegie Mellon University\\
Pittsburgh, PA 15213, USA \\
\texttt{\{yimengzh\}@cs.cmu.edu}, \texttt{\{tai\}@cnbc.cmu.edu} \\
}
